Programmable RO (PRO): A Multipurpose Countermeasure against Side-channel and Fault Injection Attack

Side-channel and fault injection attacks reveal secret information by monitoring or manipulating the physical effects of computations involving secret variables. Circuit-level countermeasures help to deter these attacks, and traditionally such countermeasures have been developed for each attack vector separately. We demonstrate a multipurpose ring oscillator design - Programmable Ring Oscillator (PRO) to address both fault attacks and side-channel attacks in a generic, application-independent manner. PRO, as an integrated primitive, can provide on-chip side-channel resistance, power monitoring, and fault detection capabilities to a secure design. We present a grid of PROs monitoring the on-chip power network to detect anomalies. Such power anomalies may be caused by external factors such as electromagnetic fault injection and power glitches, as well as by internal factors such as hardware Trojans. By monitoring the frequency of the ring oscillators, we are able to detect the on-chip power anomaly in time as well as in location. Moreover, we show that the PROs can also inject a random noise pattern into a design's power consumption. By randomly switching the frequency of a ring oscillator, the resulting power-noise pattern significantly reduces the power-based side-channel leakage of a cipher. We discuss the design of PRO and present measurement results on a Xilinx Spartan-6 FPGA prototype, and we show that side-channel and fault vulnerabilities can be addressed at a low cost by introducing PRO to the design. We conclude that PRO can serve as an application-independent, multipurpose countermeasure.

==> 01-introduction_bp.tex <==
\section{Introduction}
% {Todo-1: Yuan}
% \begin{itemize}
%   \item Side-channel leakage is threat the security of the cryptography system
%   \item What is fault and fault is another threat to the security of the cryptography system
%   \item In this paper, we introduce on a multi-functional ro-based sensor design... it has three functions including: providing side-channel countermeasure,  power sensing for real-time leakage detection, fault injection detection. 
%   \item novelty compares to existing sensor design(todo: need to check related work)
%   \item structure of this paper
  
  
% \end{itemize}

In a physical side-channel attack, an adversary learns secret information by passively monitoring or else actively influencing the implementation of a secure electronic system. While power consumption is a popular target in side-channel attacks, many other sources of physical quantities have been identified and used as side-channel leakage. Besides passive monitoring of circuit behavior, an additional cause of information leakage stems from targeted faults. By analyzing the corresponding fault response, an attacker can retrieve the secret information from a target \cite{bar2006sorcerer}. The most common methods to inject faults include power glitches, clock glitches, electromagnetic pulses, and laser pulses. Finally, fault injection and side-channel monitoring can also be used in a combined attack, for example, to break a pure side-channel countermeasure \cite{yao2018fault}. 

% \todo[inline]{add shared PDN problem -pantea}

In recent years, researchers demonstrate that the placement of the attacker and the victim circuitry on the same chip while sharing a common \ac{pdn} brings new side-channel and fault attack opportunities. Having a common \ac{pdn} intrinsically relates the perturbations from the victim's logic to the attacker's logic and vice versa. Therefore, a neighboring adversary logic can interpret information about the victim operations by monitoring the changes on the shared \ac{pdn}. On the other hand, the same physical effect exists in the other way around; The victim logic can infer malicious operations of its neighbor circuitry by monitoring the shared \ac{pdn}.



\todo[inline]{Yuan todo: add sensor requirement afterwards}

% fault-attacks actively inject well-designed disturbances, known as faults, into the systems \cite{bar2006sorcerer} \cite{yao2018fault}. The most common methods to inject faults include power glitches, clock glitches, electromagnetic pulses, and laser pulses. By analyzing the corresponding fault response, an attacker can retrieve the secret information from the system. 

% In recent years, \color{blue} physical \color{black} side-channel and fault attacks have become serious threats to the secure embedded systems. Side-channel attack is a passive non-invasive attack where the adversary can monitor and analyze the physical side effects of an electronic circuit computing on secret variables \cite{Koc96}. The physical effects typically used by attackers include power consumption, electromagnetic emission, acoustics, optical radiation, timing, etc.  By applying statistical analysis such as correlation on the leakage measurements, an adversary can derive the secret variables.  


%previous countermeasures usually only solve one problems
%
Even though many existing works have demonstrated side-channel and fault attack countermeasures, there are no simple circuit-level solutions to solve both side-channel and fault attack vulnerabilities in a generic manner, and at the same time. Generally, even for individual side-channel or fault countermeasures, a significant overhead will be introduced to the design. Moreover, many of the existing countermeasure mechanisms have to be specifically adjusted for the implemented algorithm.

Previously, \acp{ro} were widely used by silicon design houses as test structures or on-chip sensors to monitor the performance of their technologies and circuits \cite{kim2008cmos}. 
% But previous work failed to comprehensively investigate its potential in adding on-chip resistance to both side-channel and fault attacks simultaneously. 

But a multi-functional design of RO-based on-chip sensors has not been investigated in adding resistance against both side-channel and fault attacks to the circuit. 
In this work, we introduce a new multi-functional Ring Oscillator design - programmable RO (PRO). With a low overhead, the proposed PRO can provide the following solutions within the same structure: 
\begin{itemize}
    \item Active Side-channel hiding countermeasure;
    \item On-chip power monitoring;
    \item Fault detection;
\end{itemize}

\begin{figure}
    \centering
    \includegraphics[width=1.1\linewidth]{Figures/intro.png}
    \caption{PRO based on-chip Secure Network Hardware Extension}
    \label{fig:intro}
\end{figure}

The proposed PRO design has multiple configurations of oscillation frequency, which are under the control of the user (i.e., the defender). 
% Each PRO has its own counter, by comparing with a reference counter, the PRO's real-time oscillation frequency can be calculated.  
Each PRO has its own counter which can be read to calculate the PRO's frequency by comparing it with a reference counter. We first demonstrate that with low overhead, individual PRO can provide sufficient disturbance to the power to hide the side-channel leakage of the secret information in the system. Moreover, we further demonstrate that by combining multiple PROs into an array and by placing them within the module under protection, a secure on-chip monitoring network can be constructed to monitor the power fluctuations on the \ac{pdn} to detect abnormalities and fault attacks. 
%introduce the basic structure of the secure system
%it is generic to any secure module
%it 
\autoref{fig:intro} shows the overall structure of the PRO-based on-chip secure system. The PROs are evenly placed on the chip to form a secure on-chip network. The PRO secure network can be controlled by the external user configuration. The user can turn on the \ac{sca} countermeasure by configuring the PRO to oscillate at randomized oscillation frequency. The user can monitor the oscillation frequency of each PRO in the array by reading out its corresponding counter value. We demonstrate that on-chip local power attacks and EM fault injections can be detected by PRO array by monitoring the frequency change of the PROs. The proposed design can be used on any secure module, from small hardware accelerators to complex \acp{soc}. To the best of our knowledge, this is the first work to comprehensively study the potential of RO-based designs in SCA countermeasure, power sensing, and fault detection. 

The structure of the paper is as follows. The next section reviews related work of Ring Oscillators and highlights our contribution. Section \ref{sec:PRO-design} describes our proposed PRO design. In Section \ref{sec:SCA countermeasure}, we explain and demonstrate the effectiveness of PRO as a side-channel countermeasure. Next, we present the PRO's power sensing functionality in Section \ref{sec:power sensing}. We further show that PRO can detect the power fault and EM fault in Section \ref{sec:fault-detection}. Finally, we conclude the paper in Section \ref{sec:conclusion}.

\subsection{Adversary Model}
In adversary model, we defines the capability of the adversaries. In this work, PRO covers adversaries with side-channel and fault attack capabilities:\\ 
\textbf{Side-channel Attacker Model.} We consider two kinds of adversaries. First kind of adversaries have physical access to the device which enables them to control the data input and monitor the power dissipation by shunting the device's power supply. The other kind of adversaries have remote access to a shared Power Distribution Network (PDN) of the victim device and can put malicious power monitoring circuit to measure the power consumption of the device \cite{zhao2018fpga}\cite{standaert2006overview}. This enables the attacker applies side-channel attacks, such as Simple Power Analysis \cite{mangard2008power}, Differential Power Analysis(DPA) \cite{Koc96}, Correlation Power Analysis \cite{brier2004correlation}, to retrieve the secret information.\\ 
\textbf{Fault Attacker Model.} We also consider the adversaries can induce fault into the circuit by stressing the electrical environment, such as inject clock glitch, power glitch, EM glitch. These can induce targeted transient fault which can cause bit flipping, changing of the control flow of the secure algorithm, set/reset of the circuit, etc. This can be done either by exert disturbance to the circuit directly which requires adversaries have physical access to the device or has remote access to the shared cloud computing environment with the victim circuit \cite{8715263} \cite{krautter2018fpgahammer,9237147, 8844478}.   The exact fault effects to the circuit highly depends on the fault injection parameters, victim architecture, victim algorithm and fault injection techniques.  By monitoring the fault response of the circuit after injecting targeted fault, the adversaries can retrieve the secret information by performing Differential Fault Analysis (DFA) \cite{biham1997differential}, Statistical Fault Analysis (SFA) \cite{fuhr2013fault} or instruction skip attacks \cite{yao2018low}.
PRO as a secure on-chip add-on can be integrated to the circuit to protect against aforementioned attackers. Adversaries may try to tamper with the PRO sensor itself to bypass the PRO's security mechanisms, but we don't consider this adversary model within this work.




==> 09-Discussion.tex <==
\section{Discussion}

==> 11-autorbio.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{a.eps}}]%
{name}
was born in ... on ... more text.
\end{IEEEbiography}


